Towards Provable Security in Industrial Control Systems Via Dynamic Protocol Attestation

Industrial control systems (ICSs) increasingly rely on digital technologies vulnerable to cyber attacks. Cyber attackers can infiltrate ICSs and execute malicious actions. Individually, each action seems innocuous. But taken together, they cause the system to enter an unsafe state. These attacks have resulted in dramatic consequences such as physical damage, economic loss, and environmental catastrophes. This paper introduces a methodology that restricts actions using protocols. These protocols only allow safe actions to execute. Protocols are written in a domain specific language we have embedded in an interactive theorem prover (ITP). The ITP enables formal, machine-checked proofs to ensure protocols maintain safety properties. We use dynamic attestation to ensure ICSs conform to their protocol even if an adversary compromises a component. Since protocol conformance prevents unsafe actions, the previously mentioned cyber attacks become impossible. We demonstrate the effectiveness of our methodology using an example from the Fischertechnik Industry 4.0 platform. We measure dynamic attestation's impact on latency and throughput. Our approach is a starting point for studying how to combine formal methods and protocol design to thwart attacks intended to cripple ICSs.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> backups/sec_i_introduction_v1.tex <==
\section{Introduction}
Industrial control systems (ICS) are large-scale, distributed, cyber-physical systems controlled by software. Attacks on ICS software appeals to actors ranging from nation-states to hacking groups. Nation-state actors are extending the battlefield into the digital world. For example, in 2015 Russia attacked the Ukrainian power grid and disrupted service to 250,000 people \cite{cisa_alert_2016}. Meanwhile, hacking groups extract ransom payments by holding critical infrastructure at risk. Consider the 2021 Colonial pipeline ransomware attack. This attack disrupted petrol delivery to the East Coast of the United States \cite{cisa_colonial_pipeline_2023}. The consequences of attacks against ICS are severe. Thus, it is vital to secure ICS software.

Entire categories of attacks are preventable using techniques from formal methods. Formal methods are mathematically rigorous techniques to analyze the behavior of systems. Formal methods provides two popular techniques: model checking and theorem proving. Model checking exhaustively searches a system's states using a model checking tool. Model checking tools verify that each state maintains an engineer-supplied invariant. Meanwhile, theorem proving uses logic to construct a proof that a proposition holds over a model. Both approaches enable users to express and prove critical safety properties.

Model checking has proven safety properties of ICS in recent research efforts \cite{hodaOntology,modelCheckingPlcFbds,  translationBasedModelChecking, plcVerif, applyingModelChecking}. We characterize these efforts as \emph{model translation} approaches.  Model translation uses the source code of ICS software to automatically extract a formal model. A model checker can verify the model is free from safety violations. 

Model translation has three major drawbacks. First, model extraction leaves unverified software in the ICS. Detecting attacks against unverified software requires \emph{some} online monitoring. Second, researchers have reported (e.g., \cite{applyingModelChecking}) that this methodology fails to scale to large systems. Scaling is challenging because the number of states a model checking tool searches explodes as system sizes increase. Finally, model translation occurs after system implementation. If the implementation derives from a bad design then correcting defects is challenging. These drawbacks make model translation unappealing.

To address online monitoring, researchers have proposed physics-based anomaly detection  \cite{detectingAttacks, savior, bluebox, learnToRecover, realTimeAttackRecovery, roboads}. Physics-based anomaly detection identifies attacks by equipping systems with a monitor. The monitor models the physical behavior of the system using techniques ranging from Extended Kalman Filters to Deep Learning. The monitor compares the actual physical state of the system to the expected physical state. When the actual and expected states diverge the monitor reports an attack. The attack report causes the system to execute a fail-safe. Fail-safes are carefully engineered actions that ensure the system always behaves safely. However, this approach fails to consider how non-anomalous states might still be unsafe. Runtime detection must be more preventative.

% Besides model checking, developers can also show ICS software is correct using theorem proving. Theorem proving requires the use of program verification tools. Program verification tools include frama-c, Low*, and Isabelle/C \cite{framac, lowstar, IsabelleC}. Program verification tools enable compositional reasoning. Compositional reasoning uses isolated components to model systems. The system's behavior is formally specified from these components using mathematical logic. However, program verification tools are notoriously difficult to use. This difficulty renders this approach inaccessible to anyone but experts in formal methods. Yet even formal methods experts stand to benefit from an approach that reduces their efforts.

Besides model checking, engineers can also show ICS software is correct using theorem proving. Theorem proving requires the use of program verification tools. Program verification tools include frama-c, Low*, and Isabelle/C \cite{framac, lowstar, IsabelleC}. Program verification tools offer improved scaling over model checking by using compositional reasoning. Compositional reasoning uses isolated components to model systems. The system's behavior is formally specified from these components using mathematical logic. However, program verification tools lack support for describing distributed systems. This makes it challenging to prove an ICS's safety properties.

We propose developing ICS software using a new approach shown in Figure \ref{fig:overview}. Our approach enables compositional reasoning and provides support for creating distributed systems. In our approach, communication between software components occurs via remote procedure calls (RPCs). We model RPCs in an interactive theorem prover (ITP). Specifically, we use F*, a state-of-the-art ITP with sophisticated automation.  Inside F*, we embed a domain specific language (DSL) for describing communication protocols. We use our DSL to construct communication protocols that maintains the ICS's safety. We use F*'s facilities for writing mathematical logic to prove safety properties. This approach enables us to design protocols that maintain critical safety invariants.

We use automation to generate code for RPC frameworks from the DSL we have embedded in F*.  Although ITPs like F* can help verify designs, they are not suitable for writing ICS software. ICS software is often written in C and other embedded languages. The use of embedded languages makes implementing RPCs tedious. However, we can eliminate this tedium by leveraging off-the-shelf RPC frameworks. RPC frameworks use high-level message specifications to generate "boilerplate" code. With boilerplate code automatically generated, software engineers can concentrate on essential application logic.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/IntroPic.png}
    \caption{Overview of our methodology.}
    \label{fig:overview}
\end{figure}

Formally verifying all of an ICS's software components is an arduous ambition. We take up the position that it is often unnecessary. With our approach, we only need to verify software that controls physical mechanisms. For example, the low-level software that drives a servo or that opens a valve. It is easy to identify these software components. In our formal model, they make changes to the system state. Our formal proofs show that the ICS behaves safely if RPC semantics are accurately modeled; i.e., if the software that controls physical mechanisms is correct.

Despite our proofs, unverified components could still pose a safety risk if left unmitigated. For example, an adversary could compromise software in a supervisory control and data acquisition (SCADA) PC. Then, they could send commands to a programmable logic controller (PLC) that causes the ICS to behave dangerously. Moreover, unverified components might contain software bugs. Thus, even the actions of unverified components must have limited consequences. 

To mitigate the risks posed by unverified components, we propose dynamic protocol attestation. Dynamic protocol attestation involves translating the communication protocol into an automata. At runtime, the automata checks RPC calls for protocol conformance. If RPC calls do not conform to the protocol, then the checker triggers a fail-safe. Thus, the system always conforms to the protocol or executes a fail-safe. Since protocol conformance provably implies safety, the system cannot exhibit dangerous behaviors.

We demonstrate the effectiveness of our methodology in a Fischertechnik Industry 4.0 environment. Similar Fischertechnik environments have been used in previous related research efforts \cite{Cattel1996,Cattel1995,Gourcuff2008}. We use this environment to evaluate our methodology's effectiveness and performance. We show that dynamic protocol attestation imposes only a moderate overhead. 

To summarize our contributions, we:
\begin{itemize}
\item \textbf{Propose a new methodology for developing ICS software.} Our methodology enables us to construct new communication protocols in F*, a state-of-the-art ITP. We use F* to prove that protocols maintain critical safety invariants.
\item \textbf{Provide automatic techniques to translate terms in ITPs into RPC frameworks.} This generates the code necessary to create implementations of our protocol.
\item \textbf{Show how to use dynamic protocol attestation to detect protocol deviations.} 
\item \textbf{Provide experimental results that highlight the potential of our approach.} Dynamic protocol checking adds moderate overhead. In many applications, the overhead will be acceptable. Future work will consider how to further reduce the overhead.
\end{itemize}


==> backups/sec_ii_background_vaccepted.tex <==
\section{Background}

\subsection{Fischertechnik}

\subsubsection{Overview}
Industry and academia use Fischertechnik's embedded platforms~\cite{FT} to address the challenges posed by Industry 4.0~\cite{ibm_industry_4_0}.  Industry 4.0 increases the complexity and concurrency of ICS software. These increases have lead to vulnerabilities not previously found in embedded systems. Members of industry and academia are mitigating these vulnerabilities with new technical solutions, often validated on Fischertechnik's platforms.

 % One of Fischertechnik's most used platforms is the Training Factory Industry 4.0 \cite{FTfactory}.
 % %This factory is shown in Figure \ref{fig:ft-training-factory}. 
 % The provided software supports two views. The customer view allows the customer to order an item. The supplier view simulates the storage of items that will become available for purchase. The Fischertechnik items have three three different colors: red, white, or blue. The factory comes pre-programmed. However, the factory is reprogrammable. Researchers reprogram the factory to experiment with vulnerability mitigations.  

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/HBWfactory.png}
%     \caption{Fischertechnik Training Factory Industry 4.0 24V.}
%     \label{fig:ft-training-factory}
% \end{figure}

The Fischertechnik was initially used in studies involving controller verification with model checking \cite{Cattel1996,Cattel1995,Gourcuff2008,Cattel1995}, in an example implementation of model-driven systems engineering \cite{model1,model2}, and in a program analysis-based PLC code vetting study \cite{Zhang2022}. 

Researchers have also used Fischertechnik platforms to study ICS security. For example, researchers used Fischertechnik platforms to study runtime detection of improper parameters in ICSs \cite{Zhang2022}. They were also used to study decentralized monitoring of linear temporal logic (LTL) formulae \cite{Omar2021}.  Finally, a contract-based hierarchical resilience management framework which improves resilience when dealing with component failures used a Fischertechnik platform to perform its evaluation \cite{Haque2018}.

\subsubsection{High Bay Warehouse}
The Fischertechnik factory stores manufactured items in its high bay warehouse (HBW). The HBW is shown in Figure \ref{fig:ft-hbw}. The HBW provides an interface that displays items to customers. The HBW consists of nine bays that can store at most one item. The HBW interacts closely with the vacuum gripper. The vacuum grip arm delivers and retrieves items from storage. The HBW has an arm that moves items into and out of bays. We chose to implement our approach on the HBW due to its intuitive functionality and straightforward interactions with the manufacturing process and customer.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.65\linewidth]{figures/HBW.png}
    \caption{The Fischertechnik's High Bay Warehouse.}
    \label{fig:ft-hbw}
\end{figure}


\subsubsection{Critical Safety Properties}
\label{sec:safety-properties}

The high bay warehouse is vulnerable to two dangerous scenarios:
\begin{enumerate}
\item Storing a new item when the high bay warehouse is already full.
\item Attempting to retrieve an item that is not stored in a bay.
\end{enumerate}

Therefore, an ICS's software implementation must enforce three invariants. First, that the HBW is not full before it attempts to store an item. Second, that the HBW contains only processes a customer's order if it contains the desired item. Third, that the state of the bays is accurately tracked. We desire assurance that the HBW behaves safely.

\subsection{Attack Model}

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{figures/SCADAPic.pdf}
    \caption{Overview of an ICS. %The demon icon is located adjacent to components that we assume an attacker controls.}
    }
    \label{fig:attack vector}
\end{figure}

\subsubsection{Threats}
We consider a threat model where adversaries seek to compromise ICS controllers. ICS controllers are software that executes on an operating system. ICS controllers use low-level hardware drivers to manipulate the physical world. ICS controllers support emerging industry 4.0 trends by interfacing with the public internet. Interfacing with the internet jeopardizes the security of an ICS controller. Therefore, we assume an ICS controller may become compromised at any moment. Compromised ICS controllers may execute RPCs that place the ICS at-risk. 

\subsubsection{Attacker}
We assume the attacker is able to execute arbitrary RPCs on some controller in the ICS. Figure \ref{fig:attack vector} shows possible attack vectors. The attacker may use this capability to perform a lateral attack. Lateral attacks use an entry point component to compromise other components over a network. 

% If we assume this, then how can we stop it?
%We assume that attacker is able to bypass message checks. Thus, the attacker can send message sequences that would are unallowed by a security protocol.

\subsubsection{Trusted Computing Base}
We assume attackers cannot control the operating system, low-level hardware drivers, or hardware. High assurance operating systems like seL4 \cite{sel4} have formally verified security properties. These properties enable strong isolation of software components. We assume that engineers have verified the behavior of hardware drivers. We trust that hardware functions as intended. We also assume attackers have not compromised the RPC framework. We further assume the RPC framework always executes RPCs. Finally, we assume attackers have not compromised our dynamic protocol checker. 


\subsection{Interactive Theorem Provers}
Interactive theorem provers are tools that help engineers construct computer-verified mathematical proofs. Engineers write proofs in a language the ITP provides. Often, ITPs provide purely functional languages based on the Calculus of Inductive Constructions \cite{cic}. The Calculus of Inductive Constructions (CIC) is a type theory for expressing proofs. Proofs in CIC are constructed following the Curry-Howard isomorphism \cite{curryHoward}. The Curry-Howard isomorphism treats types as propositions and values as proofs. Writing a proof of a proposition amounts to writing a term whose type corresponds to the proposition. Type-checking verifies that the proof is free from mistakes in reasoning. 

ITPs provide automation that helps users write terms. Writing a term that inhabits a type is often awkward. As the type's corresponding proposition grows more complex, the situation becomes worse. To help remedy the situation, ITPs often provide tactic systems. Tactics are examples of metaprograms: programs that write programs. Tactics construct terms by exposing commands to engineers. These commands more closely match how humans think about proofs. Commands need not even be correct because the term a command produces is ultimately type-checked. Users can extend ITPs with their own tactics without compromising the soundness of their proofs.

 F* \cite{fstar} is a new ITP that makes it even easier for engineers to write proofs. Tactic systems require users to explicitly justify each step in their reasoning. But many steps in reasoning are obvious: equality is symmetric, addition is commutative, etc. Often times, humans make these steps without ever saying so. F* mimics human reasoning by integrating the Z3 SMT solver with its tactic system \cite{z3}. SMT solvers are tools that automatically prove propositions. Since it is impossible to automatically prove all propositions, SMT solvers may fail. When Z3 succeeds, an engineer is relieved of the burden. When Z3 fails, the engineer can use a combination of programming and tactics to write the proof. Z3 still fills gaps between steps, thus tremendously reducing the proof burden. 


==> backups/sec_iii_methodology_v1.tex <==
\section{Methodology}
This section describes how we construct communication protocols and prove their safety properties. Communication protocols describe legal sequences of RPCs. Ultimately, a communication protocol is a formal language inhabited by sequences of RPCs called \emph{traces}. RPCs have semantics we formally model in F*.  With our semantics, an RPC that causes the ICS to behave unsafely causes the state to become ``wrong''.  We embed a DSL for describing communication protocols in F*. Using F*, we can verify conformance to a protocol implies the ICS does not go wrong. 

However, sometimes software components meant to implement a protocol contain software bugs or are attacked. Therefore, the traces of the ICS may diverge from the protocol. To account for this possibility, we implement a dynamic protocol attestation. Dynamic protocol attestation checks that traces of the ICS conform to the protocol. Dynamic protocol attestation prevents non-conforming messages from taking the system to a wrong state.

\subsection{Fischertechnik Example}
\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/comPic.png}
    \caption{Protocol Specification}
    \label{fig:ft-example}
\end{figure}

We use the Fischertechnik factory to simulate a real world communication protocol. Figure \ref{fig:ft-example} shows the protocol. A customer can request an item of a certain color via a \lstinline{RetrieveRequest(color)} RPC. Likewise, a supplier can request to store an item using the \lstinline{StoreRequest(color)} RPC. The HBW controller receives and processes these RPCs. The effect of RPCs is contingent on the current internal state of the system. The controller can either return a rejection or an acknowledgement to the sender. The \lstinline[breaklines=true]{RetrieveRequest(color)} RPC triggers either a \lstinline{HasColor} or a \lstinline{DoesNotHaveColor} response. The \lstinline{StoreRequest(color)} RPC can trigger a \lstinline{IsFull} or \lstinline{NotFull} response. The controller then forwards the accepted requests to the low-level hardware drivers. After processing an RPC, the controller updates the current dynamic state of the the bays. 

The controller makes all policy decisions. The low-level hardware drivers faithfully execute all RPCs they receive from the controller. The safety of this communication is critically important. A controller that is either faulty or compromised can execute arbitrary RPCs. Since the protocol describes all safe executions, nonconforming traces can cause unsafe behavior. Non-conferment traces that lead to unsafe behavior are \emph{malicious traces}. A malicious trace will break at least one logical assertions defined in \S \ref{sec:safety-properties}. This can lead to outcomes such as collisions when attempting to store an item in an occupied bay. 

\subsection{DSL Design}
\input{semantics}
We describe communication protocols for the Fischertechnik using a DSL. The DSL has two components: syntax and semantics. The syntax contains RPCs, control flow primitives, and sequencing mechanisms. The DSL's semantics describe how terms in the DSL affect the ICS's state.

\subsubsection{Syntax}
The DSL makes a clear distinction between RPCs and the control flow primitives. In the DSL, RPCs are called \emph{external commands}. Control flow primitives are \emph{internal commands} that describe the system's logic. So, a trace is a concatenation of external commands. External commands are the only mechanism to modify the ICS's state. States can be valid or invalid. We represent a valid state as a pair $\sigma = \langle$ bays, input $\rangle$. $\sigma$ holds the current state of the nine bays and the current user input. We model the bays as a record of nine slots:

\begin{lstlisting}[style=fstar,frame=none,numbers=none]
type bays = { bay1 : color; ...; bay9 : color; }
\end{lstlisting}

To access each bay, we define a function:

\begin{lstlisting}[style=fstar,frame=none,numbers=none]
    bf : bays $\rightarrow$ $\mathbb{N}$ $\rightarrow$ color
\end{lstlisting}
that takes the bays and a number $n$ between 1 and 9 as arguments, and returns the current state of bay $n$.

We define a set of atomic propositions, $AP$, to reason about the internal state of the high bay warehouse. The labeling function L: state $\to 2^{AP}$ maps a state to a set of atomic propositions. An atomic proposition $p$ evaluates to true in state $\sigma$ iff $p \in L(\sigma)$.

The syntax of our DSL is: 

\[
\begin{aligned}
c &\in Color \\
ap &\in AP \\
input &\in Input \\
state &\in State \\
EC &\in Ext\_com \\
IC &\in Int\_com \\
\end{aligned}
\]

\[
\begin{array}{lll}
 c & ::= &\textbf{empty $|$ red $|$ white $|$ blue} \\
 input & ::= &\textbf{RetrieveRequest $|$ SendRequest }  \\
 state & ::= &\textbf{ $\sigma$ $|$ Wrong} \\
 EC & ::= &\textbf{ IsFull $|$ NotFull $|$ HasColor $|$ DoesNotHaveColor} \\
    & &\textbf{ $|$ Store}~ c~ \textbf{$|$ Retrieve}~ c \\
 IC & ::= &\textbf{Skip |}~ \textbf{Seq}(IC_1,IC_2)~ \textbf{| If}(ap,IC_1,IC_2)~ \textbf{|}~ EC
\end{array}
\]

To assist with the controller logic, we define the function:
\begin{lstlisting}[style=fstar,frame=none,numbers=none]
    find_color : Color $\rightarrow$ $\mathbb{N}$ $\rightarrow$ bays $\rightarrow$ option $\mathbb{N}$
\end{lstlisting}

\lstinline{find_color empty b} finds the bay that will be used during a \lstinline{Store} RPC. Similarly, \lstinline{find_color c b} finds a item colored \lstinline{c}. The function returns an \lstinline{option $\mathbb{N}$}. Values of type \lstinline{option a} are either \lstinline{Some a} or \lstinline{None}. The natural number inside the option cannot be used without accounting the possibility that the value is missing. 

\subsubsection{Semantics}
We formalize the behavior of the ICS using the semantics in Figure \ref{fig:semantics}. A state can be either a valid state $\sigma$ or an invalid state \textbf{Wrong}. A command that takes a system to a valid state is a valid command. Each command has at least two semantic rules. The first rule states the effects of performing the operations denoted by a valid command. The second rule states which commands are invalid. These rules lead the system to a \textbf{Wrong} state. Sequencing requires a third rule for evaluation of command sequences.

A trace that has reached a \textbf{Wrong} state cannot transition back into a safe state. We only accept traces that never reach \textbf{Wrong}. As an example of valid behavior, an \lstinline{IsFull} response can be sent when the bays are full. On the other hand, an \lstinline{IsFull} response sent when not all bays are not full is wrong behavior.  Such behavior indicates either a bug in the ICS or that an attacker has gained control of the ICS and is executing malicious RPCs.

Internal and external commands require different computation relations. The small-step semantics for external commands takes a state and a command and returns a new state.

\[
 \langle \text{Ext\_com,~ State} \rangle \rightarrow_{EC}   \text{State}  
\]

External commands either trigger operations that can alter the state or result in \textbf{Wrong}. The small-step semantics for internal commands also takes a state and a command. But, it must handle the sequencing of commands. It would also be valuable for it to track external commands that were already evaluated. The computation of internal commands returns: a new state, possibly another command to be evaluated, and possibly of a list of external commands.

\[
\langle \text{Int\_com,~ State} \rangle \rightarrow _{IC} \langle \text{Int\_com,~ State} \rangle.
\]

We use the $\leadsto$ notation to describe the final state a term produces. Specifically, if 
\[
\langle t, \sigma \rangle \rightarrow_{IC}
\langle t', \sigma' \rangle \rightarrow_{IC}
\ldots \rightarrow_{IC}
\langle \text{skip}, \psi \rangle
\]
we say that 
\[
\langle t, \sigma \rangle \leadsto \psi.
\]

\begin{table*}[h]
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        % Header.
        \hline
            \multirow{2}{*}{\textbf{Framework}} & 
            \multirow{2}{*}{\textbf{Overhead}} & 
            \multicolumn{3}{|c|}{\textbf{Embedded Language Support}} & 
            \multirow{2}{*}{\textbf{Custom Networking?}} & 
            \multicolumn{2}{|c|}{\textbf{Security Practices}} \\
            \cline{3-5} \cline{7-8}  &  & \textbf{C?} & \textbf{C++?} & \textbf{Rust?} &  & \textbf{Code Scanning?} & \textbf{Fuzzing?}  \\
        \hline
        Cap'n Proto \cite{capnProto} & Low & \xmark & \checkmark & \checkmark & \xmark & \xmark & \checkmark \\
        COAP \cite{coap} & High & \checkmark & \checkmark & \checkmark & \xmark & \xmark & \xmark \\
        eRPC \cite{erpc} & Low & \checkmark & \xmark & \xmark  & \checkmark & \xmark & \xmark \\
        gRPC \cite{grpc} & Medium & \xmark & \checkmark & \checkmark  & \xmark & \xmark & \checkmark \\
        \hline
    \end{tabular}
    \caption{RPC frameworks we considered adopting in our prototype.}
    \label{tab:RPC-frameworks}
\end{table*}

\subsubsection{Safety Proof}
In an unrestricted environment, both valid and invalid sequences of RPCs can be executed. To generate only valid RPCs, we restrict accepted traces to a subset of all possible traces. Our DSL introduces syntax for restricting RPCs, and underlying semantics of the RPCs.  Using our DSL, we write a term called $spec$, shown in Figure \ref{fig:spec}, that specifies a protocol. This is accomplished by pairing the atomic propositions with the If semantic rules for control flow. 

\begin{figure}[h]
\centering
\begin{lstlisting}[gobble=3, style=fstar]
   If APHasStoreRequest 
    (If APBaysFull (Is_Full)
      (Seq 
        (Not_Full)
        (If APRequestRed (Store Red)
          (If APRequestWhite (Store White)
            (If APRequestBlue (Store Blue)
              Skip)))))

    (If APHasRetrieveRequest
      (If APRequestRed
        (If APContainsRed (Seq (Has_Color) (Retrieve Red)) (No_Color))
        (If APRequestWhite
          (If APContainsWhite (Seq (Has_Color) (Retrieve White)) 
            (No_Color))
          (If APRequestBlue
            (If APContainsBlue (Seq (Has_Color) (Retrieve Blue))
              (No_Color))
            Skip)))
       Skip)
\end{lstlisting}
\caption{$spec$, the protocol specification for the HBW.}
\label{fig:spec}
\end{figure}

 

\begin{figure}
\begin{lstlisting}[style=fstar,frame=none]
#push-options "--fuel 400 --split_queries always"
let lemma_session_good ($\sigma$ : state{$\sigma$ $\ne$ Wrong}) 
  : Lemma (ensures $\sigma$ spec $\not \leadsto$ Wrong) = 
  match spec, $\sigma$ with
  | If APHasStoreRequest c1 c2, Sigma bays inputs  $\rightarrow$ begin 
    if eval_atomic_prop APHasStoreRequest $\sigma$ && eval_atomic_prop APBaysFull $\sigma$ then
      assert (None? (find_color' Empty 1 bays))
    else if eval_atomic_prop APHasStoreRequest $\sigma$ && not (eval_atomic_prop APBaysFull $\sigma$) then
      assert (Some? (find_color' Empty 1 bays))
    else if eval_atomic_prop APHasRetrieveRequest $\sigma$ && eval_atomic_prop APRequestRed $\sigma$ && eval_atomic_prop APContainsRed $\sigma$ then
      assert (mem APContainsRed (label_fn $\sigma$))
    else if eval_atomic_prop APHasRetrieveRequest $\sigma$ && eval_atomic_prop APRequestRed $\sigma$ && not (eval_atomic_prop APContainsRed $\sigma$) then
      assert (not (mem APContainsRed (label_fn $\sigma$)))
    else if eval_atomic_prop APHasRetrieveRequest $\sigma$ && eval_atomic_prop APRequestWhite $\sigma$ && eval_atomic_prop APContainsWhite $\sigma$ then
      assert (mem APContainsWhite (label_fn $\sigma$))
    else if eval_atomic_prop APHasRetrieveRequest $\sigma$ && eval_atomic_prop APRequestWhite $\sigma$ && not (eval_atomic_prop APContainsWhite $\sigma$) then
      assert (not (mem APContainsWhite (label_fn $\sigma$)))
    else if eval_atomic_prop APHasRetrieveRequest $\sigma$ && eval_atomic_prop APRequestBlue $\sigma$ && eval_atomic_prop APContainsBlue $\sigma$ then
      assert (mem APContainsBlue (label_fn $\sigma$))
    else if eval_atomic_prop APHasRetrieveRequest $\sigma$ && eval_atomic_prop APRequestBlue $\sigma$ && not (eval_atomic_prop APContainsBlue $\sigma$) then
      assert (not (mem APContainsBlue (label_fn $\sigma$)))
    else ()
    end
  | _  $\rightarrow$ ()
#pop-options
\end{lstlisting}
        \caption{Proof that $spec$ does not go \textbf{Wrong}.}
        \label{listing:proof}
\end{figure}

The proof in Figure \ref{listing:proof} verifies our safety critical property.  It takes a valid state $\sigma$ and proves that $\langle spec, \sigma \rangle \not \leadsto \textbf{Wrong}$. The proof verifies that every combination of atomic propositions allowed by $spec$ in a valid state cannot compute a \textbf{Wrong} state. Unlike other ITPs, F* can relegate the verification of boolean equations to SMT solvers. F* uses an SMT solver backend to alleviate some of the proof burden. Instead of writing hints to the proof checker, engineers write assertions they wants to verify. These assertions are encoded into SMT formulae that can be instantly verified. The proof uses the flexibility of this approach. 

\fbox{
    \parbox{0.40 \textwidth}{
      \begin{center}
          \textbf{SAFETY GUARANTEE}
      \end{center}

      Applying the small-step semantics $\rightarrow_{EC}$ to $spec$ in a state $\sigma \ne \textbf{Wrong}$ always yields a state $\sigma' \ne \textbf{Wrong}$.\\

      Formally:
      \[
      \forall \sigma \in \text{State}~ .~ \sigma \ne \textbf{Wrong} \implies \langle spec, \sigma \rangle \not \leadsto \textbf{Wrong}.
      \]
    }
}

Consider a situation where there is request to retrieve a blue item. Then, the system that follows $spec$ denies that request by sending a \lstinline{NoColor} command. The safety proof guarantees that there is no blue item in the high bay warehouse. The proof uses the the labeling function $L$ to map the current state to the atomic propositions that are true at that state. Then it uses an assert statement to ask the Z3 solver to verify APContainsBlue $\in\ L(\sigma)$. The SMT backend makes this proof style more ergonomic. There are ways to optimize the encoding. For example, the SMT solver will unroll computations a fixed number of steps. The \#push option command adds \textit{fuel} that increases the number of steps it unrolls.


% As a result, all sequences of commands generated by the specification term are safe command sequences. Thus, $spec$ generates a subset of all RPCs that cannot go wrong. Showing that $spec$ generates a trace proves the trace does not reach an unsafe state. 



To prevent illegal runtime traces from causing the ICS to go wrong, we must decide if the current trace is generated by $spec.$ We provide the implementation of a decider in F*, shown in Figure \ref{listing:decider}.

\begin{figure}[h]
\begin{lstlisting}[style=fstar,frame=none]
let rec is_trace (t : int_com) (tr : list ext_com)  (st : state) : Tot bool (decreases (length tr)) = 
   match tr with
     | []  $\rightarrow$ true
     | com :: tr'  $\rightarrow$ 
       let cmd', term', state' = eval_until_next_com st t in 
       match cmd' with
       | None  $\rightarrow$ false
       | Some com'  $\rightarrow$ 
         if None? term' then 
           com = com' && is_trace spec tr' state'
         else
           com = com' && is_trace (unwrap_some term') tr' state'
\end{lstlisting}
        \caption{Decider if $spec$ emits a trace.}
        \label{listing:decider}
\end{figure}

This decider, shown in Figure \ref{listing:decider}, compares the trace to $spec$. The decider acts as a recognizer for the safe RPC language. The decider takes the trace, $spec$, and current state as an input. As output, the decider returns true if  $spec$ generates the trace and false otherwise. The decider uses the \lstinline{eval_until_next_com} function to break down the trace into smaller command sequences. 


Given the proven safety guarantee, $spec$ cannot lead to wrong state. Given the $is\_trace$ function, it is possible to decide if a trace can be generated by the $spec$. Therefore, the following corollary holds.

\begin{corollary}
  If $spec$ generates a trace $tr$, then executing $tr$ does not cause the ICS to enter a \textbf{Wrong} state.
\end{corollary}



\subsection{Translation to RPC Framework}
We provide automation that translates terms from F* into an RPC framework. The translation occurs via procedures written using Meta-F* \cite{meta-fstar}. Meta-F* is a framework for  metaprogramming in F*. Metaprogramming involves writing procedures that write programs. Metaprogramming allows us to inspect terms in F* and emit new terms that generate code in an RPC framework. This allows us to use F* specifications to generate code for an RPC framework.

\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.49 \textwidth}
        \begin{lstlisting}[style=fstar,frame=none]
type store_response = | NotFull | IsFull
type retrieve_response = | HasColor | DoesNotHaveColor
type color = | Red | White | Blue

type hbw_rpc = {
    store_request : color $\rightarrow$ store_response;
    retrieve_request : color $\rightarrow$ retrieve_response;  
    store : color $\rightarrow$ unit;
    retrieve : color $\rightarrow$ unit;
}

let enc : encoder CapnProto hbw_rpc =
    ~\label{listing:gen_rpcs}~ _ by (gen_rpcs (`CapnProto) (`hbw_rpc))

dump enc
\end{lstlisting}
        \caption{The RPC specification in F*.}
        \label{listing:rpc-definition}
    \end{subfigure}
   \begin{subfigure}[t]{0.49 \textwidth}
        \begin{lstlisting}[style=fstar,frame=none]
interface HbwRpc {
  storeRequest @0(_0:Color) -> StoreResponse;
  retrieveRequest @1(_0:Color) -> RetrieveResponse;
  store @2(_0:Color);
  retrieve @3(_0:Color);
}

struct RetrieveResponse {
  enum V {hasColor @ 0; doesNotHaveColor @ 1;}
  v @ 0 : V;
}

struct StoreResponse {
  enum V {notFull @ 0; isFull @ 1;}
  v @ 0 : V;
}

struct Color {
  enum V {red @ 0; white @ 1; blue @ 2;}
  v @ 0 : V;
}
\end{lstlisting}
        \caption{Cap'n Proto inputs emitted from Figure \ref{listing:rpc-definition}.}
        \label{listing:capn-proto-code}
    \end{subfigure}
    \caption{Overview of the Fischertechnik's HBW RPC system.}
\end{figure*}

\subsubsection{RPC Frameworks.}
Table \ref{tab:RPC-frameworks} shows the RPC frameworks we considered adopting in our prototype. The ``Custom Networking'' column indicates if the framework supports additional network technologies. There are a large number of network technologies found in embedded systems. For example, an embedded system might use CAN, UART, SPI, and ethernet to connect its subsystems. Ideally, an embedded framework allows for extending its network layer to support these protocols.

RPC frameworks introduce overhead. Overhead originates from serializing and deserializing data. We classified overhead as either \emph{Low}, \emph{Medium}, or \emph{High}. Cap'n Proto and eRPC are low-overhead RPC frameworks. They use binary representations of data that matches how a compiler arranges data structures. This reduces overhead while serializing and deserializing data. We consider COAP to have high overhead. While COAP itself is light-weight, it is not a true RPC framework. Creating an RPC framework in COAP introduces additional overhead beyond the other RPC frameworks.

We evaluated the security practices of candidate RPC frameworks with two criteria. First, \emph{does the project use any static analysis tools?} Static analysis tools like Coverity \cite{coverity-scan} can identify vulnerabilities during development \cite{coverity-sec}. Second, we considered \emph{does the project use fuzzing?} Fuzzing is a software testing strategy that uses random inputs to try to find unexpected outputs or invariant violations \cite{fuzzing}. Fuzzing has identified thousands of defects in software \cite{fuzzing-survey, fuzzing-roadmap}. The ``Security Practices'' columns in Table \ref{tab:RPC-frameworks} reports our findings.  gRPC performed static analysis using Coverity, but stopped in 2015. Both gRPC and Cap'n Proto use fuzzing. Fuzzing is effective, having found a critical security vulnerability in Cap'n Proto in 2022 \cite{capnproto-fuzzing}. 

We  chose to initially implement support for the Cap'n Proto RPC framework based on our evaluation. Cap'n Proto is lightweight, supports many embedded languages, and has good security practices. Although Cap'n Proto does not support C, engineers can manually create C interfaces to C++ RPCs.

In the future, we plan to support additional RPC frameworks besides Cap'n Proto. Cap'n Proto lacks the ability to use common embedded networking technologies. We will eventually fill this gap using eRPC. In the long term, we plan to create our own RPC framework. We will use formal methods to prove its security properties. 

\subsubsection{Automated Translation with Metaprogramming}
Figure \ref{listing:rpc-definition}  shows F* code that describes the RPCs comprising our protocol. Critically, line \ref{listing:gen_rpcs} shows how to use our metaprogramming system. The \lstinline{by} syntax invokes F*'s tactic system. F*'s tactic system is an extensible mechanism to automate transforming terms. Individual term transformers are called \emph{tactics}. \lstinline{gen_rpcs} is a tactic that transforms an RPC framework and an F* type into an RPC encoder. RPC encoders contain code to emit inputs to an RPC framework. Emission occurs by calling the \lstinline{dump} function. Figure \ref{listing:capn-proto-code} shows the inputs that are automatically generated from the code in Figure \ref{listing:rpc-definition}.

The tactic system manipulates F*'s abstract syntax tree (AST) using \lstinline{gen_rpcs}. \lstinline{gen_rpcs} traverses the AST of the type supplied as its second argument. Several primitive types including machine integers and strings have simple, direct encodings. \lstinline{gen_rpcs} supports composite types like records by recursively applying itself to struct members. Advanced features in F*'s type system like sum types and refinement types are unsupported. 

The RPC framework's existing code generation tool transforms the framework inputs into code. We trust the RPC framework to emit correct code. The generated code contains logic to handle errors ranging from RPC cancellation to network errors. Since common errors are already handled, engineers only need to implement message semantics. 

\subsection{Dynamic Protocol Attestation}

We make no assumptions about the correctness of components implementing the RPC protocol beyond the low-level device drivers. Component defects may produce invalid traces. Thus, we introduce dynamic protocol attestation to ensure the protocol is followed at runtime. We implement dynamic protocol attestation as a proxy in C++ using Cap'n Proto, as per Figure \ref{fig:dynamic}. The proxy dynamically feeds the current trace to the decider procedure in F*. Since ICS never terminate, our approach ensures we always analyze finite traces. That is done through chopping the trace is smaller parts while keeping track of the state.

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/DynCheckPic.png}
    \caption{Dynamic Protocol Attestation.}
    \label{fig:dynamic}
\end{figure}

These checks allow the user to be sure the system is following the protocol. Consequently, it provides assurance that the system does not reach a bad state. Our approach aims to seemly introduce formal methods into the design process. It allow for the development of protocol and proofs in the same language. Thus, engineers do not need to learn multiple languages in order to secure their systems. It implements the communication scaffolding with the RPC extraction. The dynamic checker then ensures the runtime traces from the ICS comply with the protocol. Thus, any proofs written in F* hold for the implementation. For  performance reasons we implemented the procedure by hand. But, it can be automatically generated. The mechanization of the approach is left for future work.


==> z_oldsec_eval.tex <==
\section{Evaluation}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
          \hline
         \multirow{2}{*}{\textbf{Configuration}} & \multirow{2}{*}{\textbf{\textbf{Avg. Latency (ms)}}}  & \multicolumn{2}{|c|}{\textbf{Throughput}} \\
         \cline{3-4} &  & \textbf{Messages} & \textbf{KB} \\
         \hline
         Without Attestation & $0.1452 \pm 0.0007$ & 191,250 & 3,060 \\
         With Attestation & $0.1903 \pm 0.0007$ & 145,054 & 2,321 \\
         \hline
    \end{tabular}
    \caption{Numeric results from our performance evaluation.}
    \label{tab:perf_results}
\end{table}

To understand the effects of dynamic protocol monitoring on RPC performance, we conducted a performance evaluation. To perform our evaluation, we created a software implementation of the Fischertechnik HBW system. Our implementation has four components: a controller, an API, a client, and the protocol monitor. The controller models low-level physical actions. The API exposes a store/retrieve interface to the client. The client randomly sends the API messages that conforms to the API's protocol. The protocol monitor is a proxy in front of the API that verifies the messages the API sends and receives are valid. We implemented each component in C++. We implemented RPCs using Cap'n Proto with the inputs our automation generated. 

We considered two performance criteria in our evaluation. First, \emph{what is the effect on latency?} Second, \emph{what is the effect on message throughput?} We examined two measures of throughput: the number of messages sent, and the number of bytes sent. We evaluated two configurations: one without the protocol monitor enabled, and one with the protocol monitor. We evaluated each configuration for 30 seconds. Table \ref{tab:perf_results} shows our numeric results. 

There is moderate overhead imposed by protocol monitoring. Protocol monitoring increases latency by $\approx 31\%$. Similarly, protocol monitoring decreases throughput by $\approx 32\%$. Some applications may tolerate protocol monitoring's performance overhead. Performance overhead can be reduced in future work.

\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.49 \textwidth}
    \includegraphics{figures/cdf_plot_no_monitoring.pdf}
    \caption{Without Attestation.}
    \end{subfigure}
    \begin{subfigure}[t]{0.49 \textwidth}
    \includegraphics{figures/cdf_plot_monitoring.pdf}
    \caption{With Attestation.}
    \end{subfigure}
    \caption{CDFs of message latencies.}
    \label{fig:monitoring_cdf}
\end{figure*}

To better understand protocol monitoring's impact on latency, we examined the CDFs of our two evaluation configurations. The CDFs are shown in Figure \ref{fig:monitoring_cdf}. We observe that protocol monitoring preserves the shape of the original CDF. In particular, $99^{\text{th}}$ percentile latency also increases by $\approx 30\%$. Despite this increase, it is promising that protocol monitoring's worst-case performance appears tied to its average-case performance.
